Learning Linear Policies for Robust Bipedal Locomotion on Terrains with Varying Slopes

In this paper, with a view toward deployment of light-weight control frameworks for bipedal walking robots, we realize end-foot trajectories that are shaped by a single linear feedback policy. We learn this policy via a model-free and a gradient-free learning algorithm, Augmented Random Search (ARS), in the two robot platforms Rabbit and Digit. Our contributions are two-fold: a) By using torso and support plane orientation as inputs, we achieve robust walking on slopes of up to 20 degrees in simulation. b) We demonstrate additional behaviors like walking backwards, stepping-in-place, and recovery from external pushes of up to 120 N. The end result is a robust and a fast feedback control law for bipedal walking on terrains with varying slopes. Towards the end, we also provide preliminary results of hardware transfer to Digit.

==> Sections/Introduction.tex <==
\section{Introduction}

%\textbf{need to change this paragraph}
%Over the last few years, there has been a surge in the development of low-cost and open-source quadruped robots \cite{Nathan2019Stanford}, \cite{grimminger2019open}, \cite{dhaivatdesigndevelopment}.
%Due to limitations in actuation/sensing capabilities, developing a control law that yields stable walking in these types of robots is cumbersome. Some of these robots do not possess 
% foot contact sensors for stance-swing phase detection \cite{Nathan2019Stanford}, \cite{grimminger2019open}, and 
%BLDC motors for accurate torque control \cite{dhaivatdesigndevelopment}. In addition, deployment of some of the advanced control laws like the model predictive control (MPC) \cite{Kim2019HighlyDQ}, Deep Neural Networks (DNN) \cite{google_paper,Hwangboeaau5872} require expensive computational resources.
% ) as opposed to series elastic or hydraulic actuators ,and do not possess foot contact force sensors or force torque sensors. Developing a controller for such robot hardware is a time consuming task that requires extensive domain knowledge and tedious manual tuning. 
%Therefore, in this paper, we would like to answer the following question: What is the minimum possible control framework that can be deployed to realize stable locomotion behaviours in medium-size low-cost quadruped robots? % with servo motors and limited sensing capabilities?

Locomotion for legged robots has been an active field of research for the past decade owing to the rapid progress in actuator and sensing modules. 
Actuators like the BLDC motors are more efficient and powerful, and sensors like the IMUs are more accurate and affordable.
% Efficient actuators via the servo drives
As a result, there is a spurt in the growth of high performance legged robots  \cite{DBLP:journals/corr/abs-1803-05580,Bledt2018MIT,Hwangboeaau5872}. In particular, there has been rapid progress in the domain of quadrupedal robots, and there a general push for realization of natural and efficient locomotion behaviors that are comparable with animals.
%motion primitives because most of their motion primitives have been derived from naturally occurring animal movement strategies. 
% The most advanced robots aimed at achieving human motion are bipedal robots and humanoids. 
While the bipeds and quadrupeds of today are able to perform highly dynamic behaviors, 
the corresponding controllers developed are complex.
% the effort exerted by them to plan associated motor tasks is non-negotiable. 
%Various research works have demonstrated the use of repetitive strategies and reduced parameters to define specific paths. 
% 
% For example, the MIT Cheetah uses Model Predictive Control (MPC) with Raibert's torso regulation \cite{Bledt2018MIT}, the ANYmal robot uses Neural Network policies trained via .
In this context, most of such works have focused on quadruped robots accompanied by the inherent advantage of balance. %on more than one passive leg. 
However, bipedal robots, having a single supporting leg, suffer from a loss of balance and stability. A lot of works for quadrupeds \cite{Lee_2020}, \cite{gangapurwala2020rloc} have shown robust locomotion over rough terrains through learning but none have extended their approaches to the other class of legged robots. Although there are unified frameworks for multi-legged systems, strategies working for quadrupeds seldom transfer directly to bipeds without heavily engineered, complicated regulations. For example, MIT Cheetah \cite{Bledt2018MIT} uses a single rigid body model of the system for the walking controller, which does not hold good for bipedal systems. Hence, there is a dire need for a unified framework that can generalize among legged robots yet is simple and scalable enough to implement in any bipedal robot. 
%For example, MIT Cheetah \cite{Bledt2018MIT} uses single rigid body model for the walking controller, but the bipeds cannot be considered as a single rigid body. Hence, there is a dire need for a unified framework that can generalize among legged robots yet is simple and scalable enough to implement in any bipedal robot. %skip complex dynamics and intermittent interactions with the environment.

%The domain of bipedal walking has reached maturity today, with a slew of robots developed and deployed worldwide \textbf{cite some bipedal robot papers}. 

%The domain of quadrupedal locomotion has reached maturity today with quite a few research labs/companies successfully commercializing their quadrupeds. A slew of techniques are in use---inverted pendulum model-based controllers \cite{raibert1986legged}, zero-moment point- based controllers \cite{vukobratovic2004zero}, hybrid zero dynamics \cite{hzd_grizzle}, model predictive controllers \cite{Kim2019HighlyDQ}---to name a few.
%However, these techniques are not suitable for our goal because they require extensive domain expertise.
%The long term goal of our work is to create a quadruped controller akin to inexpensive flight controllers developed for remote piloting of autonomous aircrafts \cite{pixhawk2011,px42015}. The difficulty in developing such a controller is that it must be capable of adapting to different quadruped robots with minimum modifications. %, %on a low-cost embedded hardware,
% and simultaneously adhering to the constraints of the said quadruped robot.

%\begin{figure}[t!]
%\centering
%%\vspace{2mm}

%\includegraphics[height = 0.7\linewidth] {Figures/BipedImages/dig_rab_intro.png}
%    \caption{Temporary, will make it more proportional}
%\label{fig:IK_S2}
%\vspace{-2mm}
%\end{figure}

\begin{figure}[!t]
\centering
%\vspace{2mm}

\includegraphics[width = \linewidth, height = 7cm]{Figures/BipedImages/intro_train_3.png}
\caption{Figure showing Rabbit (Top) and Digit (Bottom) in Simulation: Traversing incline and decline with robustness towards adversarial forces}
\label{fig:intro_train}
\vspace{-5mm}
\end{figure}


%Bipedal locomotion with a library of gaits has been successfully demonstrated via numerous techniques---inverted pendulum model based controllers \cite{raibert1986legged}, hybrid zero dynamics \cite{8815085}, central pattern generators \textbf{can cite the paper from Italy} \cite{6739463}---to name a few. 
%However these techniques are not suitable for our goal .... 
%because they are heavily model-based and require extensive knowledge of the robot system modeling. In other words, customized control laws are required for realizing stable walking gaits in hardware.
% However these techniques are not suitable for low cost quadruped robots because they tend to require expensive sensors such as IMU's, actuators that have torque control capabilities,
% (Improve the citations here, not relevant enough)
% (\cite{raibert1986legged}-\cite{Kim2019HighlyDQ}), large amounts of computation (\cite{Kim2019HighlyDQ}, \cite{Hwangboeaau5872}) or extensive domain knowledge and tuning (\cite{hzd_grizzle}, \cite{ijspeert2008central}). 
%With a view toward ``automatically" developing control algorithms for a broad set of servo driven quadruped robots, 
%As shown in \cite{paigwar2020robust}, we aim to learn a simple policy that outputs the end-foot reference trajectories that can be tracked by the individual joints, resulting in stable walking.
%To this end, data driven approaches like
%Reinforcement Learning (RL)  \cite{kober2013reinforcement}, which are capable of learning walking controllers by themselves 
% that directly map from the states the robot can measure (e.g. motor angles) to the actions the robot can perform (e.g. position control of motors) 
%seem very attractive. 
% In our formulation, we learn a linear policy, i.e. a single matrix which can be implemented on microcontroller based hardware boards (like the STM32 series or ARM Cortex M4 series) using RL and is capable of traversing slopes, rough terrain and rejecting disturbances. 
% Having trained an optimal policy specific to the quadruped with appropriate reward models, 
 
 % vWe will show that this approximation does not affect the quality of the gaits inferred by comparing the efficiencies.
% Appropriate gaits such as turning, trotting are chosen based on an external user command.
% and transition between them to demonstrate a wide variety of locomotion patterns. 
% On this note, the main contribution of this work is in introducing a framework by which a user can upload the description of his quadruped robot and quickly generate an omni-directional controller which can then be implemented on an off the shelf low cost micro-controller like an Arduino. We to use this framework to test and develop a controller for our in house quadruped robot Stoch2.




% The considerable success shown by D-RL are mostly for simulated robotic tasks \cite{kober2013reinforcement} even today. Translating these results in real hardware are faced with numerous challenges. 
% The use of deep neural networks (DNN) entails a large computational overhead to obtain an inference. This inference may not possible to obtain in real-time but even when possible requires expensive hardware and high power consumption, which may not be economical for a large commercial deployment of robots.
% In addition, standard D-RL based techniques require a significant number of training iterations (to the order of millions) which again requires large compute power and time, can only be done in simulation often requiring extensive reward engineering that can take weeks to perfect.\
% In contrast in our proposed method we show that by training multiple shallow neural networks and transitioning between them we can obtain robust control policies, that can be run on standard inexpensive micro-controllers, requires comparatively very less training time and compute power to generate, and learns with simple shaped reward functions. 
% A possible alternative would be to train in a simulated environment, and then deploy on hardware. This was demonstrated by \cite{google_paper}, \cite{Hwangboeaau5872}, \cite{xie2019iterative} for quadrupeds and bipeds, where the neural networks used sensory feedback to control the motor joints in real-time. However, this type of sim-to-real transfer presents with itself several challenges. Some of these challenges are mainly attributed to the modeling uncertainty, sensory noise, control saturations etc. 





%Researchers have tried to eliminate the extensive manual tuning and expertise required by using evolutionary strategies and reinforcement learning  \cite{singla2018realizing}.  
% It is worth noting that some of the solutions to the above presented challenges were addressed in part via the traditional RL techniques \cite{Hornby1999Autonomous,quinlan2003techniques,kohl2004policy,tedrake2004stochastic}. In fact, RL was used as an optimization tool (gait generating tool) by most of the teams participating in the quadruped RoboCup soccer league in 2004 as stated by \cite{Chalup2007Machine}. These techniques have been used to obtain the parameterized  foot trajectories that can be deployed on the robot. This can be implemented in low cost hardware and requires no extra computing power. However, these works implemented open-loop controllers to playback the trajectories on the robots, thereby, limiting their capability to handle external disturbances due to lack of feedback in the system.  


% Similar to the methodologies followed in the past in RL, we would like to realize locomotion on a low-cost embedded platform and, at the same time, incorporate some form of feedback that will help improve robustness in real-time. By limiting our controller to a linear policy, i.e., a single matrix with no activation functions, our goal is to learn this policy with the modern tools available for learning. We chose to use a model-free and gradient-free algorithm, Augmented Random Search (ARS), which was shown to be at least as sample efficient as DNN based policy gradient algorithms \cite{mania2018simple} existing in literature. 
% We present a control architecture that combines a trajectory-based framework with RL to obtain a controller that is capable of handling external disturbances and exhibiting multiple complex quadruped locomotion behaviours while requiring little manual tuning. 

% \subsection{Related work on quadruped control}

%\subsection{Related work}

%\textbf{Bipeds are very hard, quadrupeds are easier, in simulation there are unified frameworks for bipeds, quadrupeds, but in experiments whatever worked for qadurupeds dont apply to bipeds. For example, MIT Cheetah \cite{Bledt2018MIT} uses single rigid body model for the walking controller, but th ebipeds are not single rigid body.
%various methods used for bipeds: SLIP models, rabiert's controller, MPC, HZD: there is a lot of mix and match. We would like to use the strength of learning to determine the linear policies. (from the learning point of view it is straightforward).}

Correspondence between one-legged hopper, biped, and quadruped gaits to produce locomotion policies that share significant structure was first explored by \cite{raibert1986legged}. Since then, the sub-classes of quadruped robots gained popularity due to their implicit balancing ability. Various works have contributed on making physically realizable motions in bipeds with centroidal models like ZMP \cite{tedrake2015} and SLIP \cite{apgar2018rss}. In this context, dynamics based trajectory optimization \cite{xiong2018ames} and tracking controllers based on quadratic programming \cite{heried2018cfrost} or feedback linearization \cite{gongetal2018} are well known. Model Predictive Control (MPC) \cite{powell2015icra}, and Hybrid Zero Dynamics (HZD) \cite{hzd_grizzle} modelling the underlying dynamics more accurately, tend to yield more natural dynamic walking behaviors. \cite{da2019grizzle} blended the concepts mentioned earlier with learning algorithms to control the high dimensional bipedal system based on a low-dimensional surface of the system's state space. Recently, \cite{gong2020angular} utilizes the simplified Angular momentum-based LIP controller to achieve agile walking on irregular terrains with significant elevation (wavefield). 
However, unlike the robot used in \cite{gong2020angular}(Cassie), robot platforms discussed in this work have significant torso inertia and require separate terrain relative torso adaptation strategies.

%This paper aims to advance our framework in quadrupeds \cite{paigwar2020robust} to high dimensional bipeds without the loss of generality. %We revisit kinematic planning-based strategies\textbf{cite old kinematic papers} to develop task space trajectories and modulate them using recent reinforcement Learning (RL) approaches for robust training and dynamics approximation. 
%The proposed approach claims a unified framework for developing robust locomotion strategies for multi-legged robots.

%\cite{morimoto2004cmu} first explored RL for bipedal walking where traditional Poincare map of the periodic walking pattern was analyzed and tracked through PD servo controller. 
%They learned the phase and frequency of the gait to estimate the end-foot trajectories. 
%Shortly after, \cite{tedrake2004} explored 3D walking with a policy gradient-based controller working on a passive dynamic walker model and reduced actuation space. 
%Since then, various works have depicted RL algorithms' role as a replacement for various optimal control theory approaches. 
%While they suffer from sample inefficiency and are over-parametrized, the estimation of the system dynamics employing non-linear neural network formulations saves from dynamic modeling inaccuracy and inconsistency errors.
Reinforcement Learning (RL) has been quite popular as a replacement for various optimal control theory approaches as highly non-linear neural network-based deep reinforcement learning (DRL) strategies came up with interesting results.%We would like to explore the strength of learning in this work.
Physics-based bipedal character animation has thrown lights on various advantages of such DRL algorithms by generating robust locomotion strategies for rough terrains \cite{cdmloco}. Such methods ensure that the policy converges to a more practical solution using reference trajectories  \cite{deeploco} and have not yet shown to be suitable for physical robots. Usage of such reference motions \cite{RoboImitationPeng20} or a non-random sub-optimal initial policy could significantly leverage the sample efficiency and reduce the burden on the learning algorithm. However, obtaining such reference motion could be tiresome, and the development of sub-optimal initial policies through behavioural cloning \cite{paigwar2020robust} is not straightforward and is often as difficult as the learning itself. In this context, \cite{cassie2019sim2real} used a DRL framework for walking on flat terrain and presented a direct policy transfer from generating learned strategies from simulation to a physical robot. Such DRL-based policies are computationally intensive and were unable to generalize to rough terrain walking. Recently, \cite{guillermo2D, guillermo3D} introduced HZD based RL framework for developing robust flat ground walking using small scale neural networks. Unlike any of the previous works on flat ground walking, slopes and elevated terrains impose a new set of challenges, which shall be our primary focus in this paper. To our knowledge, our work is the first to demonstrate robust bipedal walking on inclined planes with the most compute-efficient control policy (which is linear) obtained through reinforcement learning. 
% \textbf{add linear RL and a good conclusion}

%In order to make physically realizable motions, various works have been using centroidal models like ZMP \cite{tedrake2015} whereas various others use SLIP to simplify the robot dynamics \cite{apgar2018rss} for faster planning. To utilize the full dynamics of the robots, trajectory optimization \cite{xiong2018ames} is used to generate trajectories, and tracking controllers based on quadratic programming \cite{heried2018cfrost} or feedback linearization \cite{gongetal2018} can be designed along them. Model Predictive Control (MPC) \cite{powell2015icra}, and Hybrid Zero Dynamics \cite{hzd_grizzle} model the underlying dynamics more accurately, which yields more natural dynamic walking behaviors. \cite{da2019grizzle} blends the concepts mentioned earlier with learning algorithms to control the high dimensional bipedal system based on a low-dimensional surface of the system's state space. Recently, \cite{guillermo2D, guillermo3D} introduced HZD based RL framework for developing robust flat ground walking using small scale neural networks. 
%Slopes and elevated terrains impose a new set of challenges to bipedal locomotion. 
%\cite{paigwar2020robust}, briefly discusses the foot placement strategies available for quadruped locomotion on slopes. 
%Recently, \cite{gong2020angular} utilizes the simplified Angular momentum-based LIP controller to achieve agile walking behaviours on irregular terrains with significant elevation (wavefield). 
%However, unlike the robot used in \cite{gong2020angular}(Cassie), both the robot platforms discussed in this work have significant torso inertia and require separate terrain relative torso adaptation strategies.

%Reinforcement learning (RL) for quadrupedal walking was first explored by \cite{kohl2004policy}, where policy gradient algorithms were used to learn optimal parameters for end-foot trajectories. The learned trajectories were then tracked in each foot in open-loop.
%However this controller was an open-loop controller, not reactive to feedback. 
% Since then research effort has gone into realizing controllers with feedback through learning techniques.

%A deep reinforcement learning framework (D-RL) was used in \cite{Hwangboeaau5872}, \cite{Jie2018Sim},  for training a deep neural network (DNN) based feedback policy for walking on flat terrains by first training the policy in simulation, and then bridging the sim-to-real gap with domain randomization and motor-modelling. 
%\cite{Jie2018Sim} first demonstrated a deep reinforcement learning (D-RL) based feedback policy for straight line walking by first training the policy in simulation and then bridging the sim-to-real gap with domain randomization and motor-modelling. %We have used the same techniques to bridge the sim-to-real gap. 
% In \cite{singla2018realizing}, motion primitives were extracted from the learnt trajectory to bridge the sim-to-real gap. 
%\cite{Hwangboeaau5872} trained a deep reinforcement learning network capable of tracking arbitrary linear and angular velocities of the center of mass on a flat terrain while \cite{jain2019hierarchical} trained a hierarchical reinforcement learning network to do the same. 
%However, these DNN based policies are computationally intensive and were unable to 
% do not 
%generalize to rough terrain walking. Similarly \cite{PMTG}, \cite{Trajectory2019Kolathaya}, \cite{Sashank2020Gait}  trained a quadruped for a flat terrain, where the learning process was sped up significantly by parameterizing the control policy using central pattern generators, B\'ezier curves and rational B\'eziers respectively. In our paper, we also parameterize our control policy with elliptical curves to speed up training. \cite{rajeswaran2017towards} first demonstrated the capabilities of a linear policy for robotics control in simulation while \cite{tirumala2019gait} used the linear policy approach to create policies for flat terrain quadruped walking. We also use a similar linear policy paradigm for rough terrain quadruped walking.  % Training a quadruped to walk on a rough terrain is a much harder problem and combining domain expertise with learning techniques seems promising. 
%Walking on arbitrary terrains was formulated as a nonlinear optimization problem in \cite{winkler18}. \cite{melon2020reliable} learnt the parameter initialization for the above nonlinear optimization problem, improving the accuracy and speed of the optimization and enabling the quadruped robot to navigate bumpy terrain. We used a similar initialization technique in our training process. A custom RL algorithm was used in \cite{Tsounis2020Deep},  to enforce footstep constraints in order to train walking over stairs, slopes and ridges. Similarly \cite{Kolter2007Hierarchical} uses hierarchical apprenticeship learning and expert data to navigate a rocky terrain. 
%However, these policies %is only capable of walking, not trotting and 
%require a complete terrain map of as an input to work. Our focus is mainly in trotting on slopes %with $0^\circ-11^\circ$ inclines 
%with  proprioceptive feedback. 

%Outside of learning, a large number of techniques have been developed to navigate a rough terrain for a quadruped robot in a blind manner. The MIT Cheetah robot achieved this by using Model Predictive Control for the stance legs and Raibert's controller for the swing legs \cite{Bledt2018MIT}. Similarly, \cite{Dario2017Dynamic} demonstrated a hierarchical blind whole body controller for the Anymal robot. However, these techniques require expensive Series Elastic Actuators or Quasi Direct-Drive actuators in order to function. In contrast, our approach requires only hobby servo motors and mainly focuses on reinforcement learning for rough terrain locomotion. 

%These works are parallel to our work, where we focus on reinforcement learning applied to walk on a rough terrain. 


% % Reinforcement learning algorithms 
% Some of these algorithms are Trust Region Policy Optimization \cite{schulman2015Trust}, Proximal Policy Optimization \cite{Schulman2017ProximalPO}, Soft Actor-Critic algorithms \cite{Haarnoja2018LearningTW}.
% Some of the methodologies followed to address the sim-to-real gap such as domain randomization, motor modeling were novel that resulted in robust locomotion in hardware.
% Since the training iterations are of the order of millions, training was always in simulation, which required accurate physics models in the simulator. However, translating gaits learned from these techniques require heavy computational resources. Therefore, with a view towards simplicity that was followed in the earlier literature \cite{tedrake2004stochastic}, we aimed to obtain optimal end-foot trajectories for the robot with the modern tools available today. In fact, we have used an augmented version of random search algorithms (called the ARS), which are known to be $15$ times faster than TRPO, PPO algorithms \cite{mania2018simple}. ARS is primarily used for training linear policies for robotic systems \cite{mania2018simple}. This algorithm was successfully demonstrated on the simulated MuJoCo robot control tasks to obtain rewards that were on par with the rewards obtained by deep nets trained using traditional Reinforcement Learning Algorithms like TRPO and PPO \cite{mania2018simple}.

% Trajectory based policy search algorithms have been recently used in 
% \cite{Trajectory2019Kolathaya} to obtain low dimensional trajectories for forward trotting. Similarly \cite{PMTG} trained a deep neural network to modulate a trajectory generator as opposed to directly learning the motor currents. This significantly reduced the training time and was capable of controlling the velocity of the quadruped robot along a straight line. Jain et al. \cite{jain2019hierarchical} extended the above work enabling limited turning motion on the quadruped robot using hierarchical reinforcement learning. These approaches produced impressive results and are closest to the work presented in this paper

\subsection{Contributions and Paper Organization}

The primary contributions of the paper are as follows:

\textbf{Low computational overhead:} The main contribution of this paper is on training robust bipedal walking on challenging terrains with low computational footprint. By incorporating the priors of bipedal walking strategies and formulating a relevant control structure,  we significantly decrease the number of learnable parameters to  9 for Rabbit (2D) and 80 for Digit (3D). Our linear control policies are considerably compact compared to even the smallest of the neural network policies \cite{castillo2019hybrid} capable of 3D bipedal walking. We firmly believe that having such a simplistic linear policy will greatly leverage our policy's explainability compared to any of the previous works, \cite{xie2019iterative}, \cite{cassie2019sim2real}, \cite{siekmann2020learning}, \cite{duan2020learning}. This feature allows us to obtain intuitive seed policies that enhance the sample efficiency of learning and realization of practical walking behaviours.

\textbf{Unified framework:} We previously achieved robust locomotion via linear policies in quadrupeds \cite{paigwar2020robust}.  Given the success behind this policy, we focused on implementing this methodology in bipeds, which are much harder to control. More importantly, bipeds have feet, which play a major role in stabilizing the torso. We have a unified learning-based linear control framework deployed alike for both quadrupeds and bipeds. 

\textbf{Robustness and generalization:} We demonstrate walking on slopes of up to $20\degree$, walking backwards, and with feet. Our controller can reject disturbances, adapt to terrain transitions, and recover from adversarial force perturbations up to $120$ N. We validate our results on two bipedal robots, Rabbit and Digit, in simulation and show preliminary transfer of the policies in Digit hardware.

% Our approach consists of a feedback control to dynamically shape these trajectories based on the body and plane orientation. Semi-elliptical trajectories parameterized by time are tracked by the individual feet. These semi-elliptical trajectories are ``shaped" by using feedback, i.e., the step-length, position and orientation of these trajectories are varied via a linear feedback policy. The policy takes the torso orientation and terrain slopes as inputs, and outputs the parameters in real-time.


% We previously achieved robust locomotion via linear policies in quadrupeds \cite{paigwar2020robust}. In this work, the goal was to focus on development of controllers for low-cost hardware. Given the success behind this policy, we focused on implementing this methodology in bipeds, which are much harder to control. More importantly, bipeds have feet, which play a major role in stabilizing the torso. This is the main focus in this paper. We demonstrate walking on slopes of upto $20$ degrees, walking backwards, and with feet.

% Our controller is capable of rejecting disturbances and maintaining balance on slopes of various inclines. %It uses body orientation and the slope angle as feedback. 
% The support plane is estimated using forward kinematics and foot contacts similar to \cite{Bledt2018MIT}. We also restrict our policy to being linear. This linearity requires low computation, thus enabling our policy to be run in real-time on an on-board embedded system. Augmented Random Search (ARS), a well-known algorithm for training linear policies \cite{mania2018simple}, is used to learn our proposed policy. We validate our results on the indigenously developed quadruped robot, Stoch $2$ in simulation. %, and video results are provided in the supplemental material.

% 1) Real-time feedback control via linear policy
% 2) Walking on terrains with varying slopes.
% 3) Disturbance rejection (robustness to pulls-pushes
% 4) Cheap hardware simple control template


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Organization}

%The paper is structured as follows: Section \ref{sec:background} will provide a description of the robots Rabbit and Digit, and the associated control framework, Section \ref{sec:learningalgorithm} will describe the training process used. This will be followed by simulation results in Section  \ref{sec:results}.

The paper is structured as follows: Section \ref{sec:background} will provide the description of the robot test-beds and the associated hardware considerations. Section \ref{sec:approach} will describe the control framework for the proposed strategy, followed by the description of the training process used, in Section \ref{sec:training_eval}. Finally, the simulation results and preliminary transfer of the framework to hardware will be discussed in Section \ref{sec:simulation_results} and Section \ref{sec:conclusion} respectively.

